Empowering Cognitive Digital Twins with Generative Foundation Models: Developing a Low-Carbon Integrated Freight Transportation System

Effective monitoring of freight transportation is essential for advancing sustainable, low-carbon economies. Traditional methods relying on single-modal data and discrete simulations fall short in optimizing intermodal systems holistically. These systems involve interconnected processes that affect shipping time, costs, emissions, and socio-economic factors. Developing digital twins for real-time awareness, predictive analytics, and urban logistics optimization requires extensive efforts in knowledge discovery, data integration, and multi-domain simulation. Recent advancements in generative AI offer new opportunities to streamline digital twin development by automating knowledge discovery and data integration, generating innovative simulation and optimization solutions. These models extend digital twins' capabilities by promoting autonomous workflows for data engineering, analytics, and software development. This paper proposes an innovative paradigm that leverages generative AI to enhance digital twins for urban research and operations. Using freight decarbonization as a case study, we propose a conceptual framework employing transformer-based language models to enhance an urban digital twin through foundation models. We share preliminary results and our vision for more intelligent, autonomous, and general-purpose digital twins for optimizing integrated freight systems from multimodal to synchromodal paradigms.

==> Sections/999-backup.tex <==
The global freight transportation sector, which includes road, rail, and waterway transport, plays a significant role in contributing to greenhouse gas (GHG) emissions, accounting for approximately 11\% of global emissions \citep{international2012co2}. In the United States, the transportation sector alone was responsible for a substantial share of national emissions, contributing 38\% of the country’s energy-related emissions in 2021, amounting to 4.6 billion metric tons of carbon dioxide \citep{shirley2022emissions}. These figures underscore the profound impact of freight and logistics on climate change and emphasize the necessity for innovative and sustainable approaches to mitigate emissions. Beyond direct carbon emissions, the transportation sector has been profoundly affected by recent global disruptions. The COVID-19 pandemic, in particular, exposed vulnerabilities within cargo transportation networks, highlighting the urgent need for resilience and adaptability in freight logistics \citep{golan2020trends}. This crisis emphasized that ensuring the robustness and efficiency of global supply chains is not only an economic imperative but also a matter of social and environmental sustainability. Addressing these challenges requires reevaluating how freight transportation systems are designed and managed to cope with such disruptions in the future. A critical component of logistics networks, intermodal freight transportation has emerged as a foundational element of modern supply chain management. Intermodal transport involves the movement of goods from origin to destination using multiple modes of transportation, such as trucks, trains, and ships, without the handling of the cargo itself when changing modes \citep{turbaningsih2022multimodal, kengpol2014development}. By leveraging the strengths of different transportation modes, intermodal freight aims to optimize operational efficiency, reduce costs, and minimize the environmental impact of cargo transport. It offers significant potential for reducing carbon footprints by enabling better route planning, consolidating shipments, and utilizing more energy-efficient modes of transportation, such as rail and waterways, for long-distance hauls. 

Despite its operational efficiency, managing an intermodal freight transportation system presents numerous methodological challenges. These challenges necessitate a comprehensive decision-making strategy to identify the most optimized transportation approach between specific Origin-Destination (OD) pairs within a real-world supply and demand context. Such an approach often requires combining different transportation modes and routes to minimize delivery times, reduce operational costs, and lower greenhouse gas (GHG) emissions, while also ensuring the seamless transition of goods across diverse transportation methods and socio-economic environments \citep{aljadiri2023evaluating}. At the methodological level, achieving efficiency in intermodal freight systems is hindered by the complexity and uncertainty inherent in real-world logistics. The transportation network is characterized by interconnected and sophisticated process dynamics, including the movement, storage, deconsolidation, consolidation, intermodal transition, and handling of shipments and containers \citep{lv2019operational, reis2019intermodal}. Furthermore, each mode of transportation is subject to unique constraints, which can vary significantly across different geographic areas. The intricate nature of these processes is further compounded by constantly changing factors such as traffic conditions, extreme weather events, and unforeseen accidents—all of which introduce an additional layer of uncertainty to decision-making. In addition, developing a sustainable optimization strategy for intermodal freight transportation systems requires complex and time-consuming technical efforts. Such strategies often involve processing large volumes of diverse urban data, coupled with simulations to monitor and predict dynamic processes throughout the supply chain. Moreover, the development of sophisticated mathematical optimization algorithms is crucial to determining the best combination of transportation modes, routes, and operational practices from millions of potential alternatives, based on a variety of constraints and objectives. 

In recent years, industry and academia have increasingly adopted digital twin approaches to enhance data- and simulation-driven processes for intermodal optimization. By leveraging advanced ICT and 5G networks, digital twins—virtual replicas of physical systems—allow stakeholders to monitor, simulate, and optimize intermodal operations in real time. Integrating traffic sensors, GPS data, freight simulations, and machine learning models, digital twins help predict disruptions, evaluate operational scenarios, and identify the most efficient strategies, thereby improving resilience, flexibility, and sustainability in supply chains. Building on existing practices in urban digital twin development for situational awareness, predictive analytics, and decision support, this vision explores how emerging generative AI technologies can address the technical and methodological challenges in creating intelligent and efficient digital twins for intermodal freight systems. Inspired by multimodal and multi-agent systems, this paper proposes a generative foundation model approach, powered by transformer-based language models, to automate data engineering and software development for prototyping digital twins. This work highlights an automated knowledge graph-driven approach for digital twin feature creation and analytics. We demonstrate initial results of this prototyping foundation model, using emerging embedding, vector databases, and retrieval-augmented generation (RAG) techniques. Additionally, we share insights on integrating these foundation models with conventional software engineering practices within a digital twin platform.

\citet{busse2021towards} presents a Digital Supply Chain Twin (DSCT) as a comprehensive solution for optimizing multimodal supply chains, which face challenges due to their complexity and lack of transparency. The DSCT is a dynamic simulation model that provides real-time visibility across the entire supply chain by integrating data from various logistics actors, such as freight forwarders, shipping companies, and terminal operators. By creating a digital replica of the physical logistics system, the DSCT can simulate different scenarios, enabling stakeholders to evaluate the impact of disruptions, optimize resource allocation, and improve decision-making processes. The DSCT leverages technologies like the Internet of Things (IoT), 5G, cloud computing, and artificial intelligence to ensure real-time data flow and predictive analytics, allowing for the synchronization of diverse transport modes, including road, rail, and maritime. This approach supports freight transportation by enhancing operational efficiency, reducing lead times, and increasing the resilience of supply chains. The DSCT not only focuses on economic and reliability improvements but also contributes to ecological sustainability by promoting better utilization of transport resources, making the overall supply chain more adaptive and efficient.

\citet{issa2024railway} introduces a Digital Twin (DT) for the railway system as an innovative tool to support multimodal freight transportation, focusing on enhancing collaboration between different stakeholders within the transport sector. The Digital Twin, developed at SNCF Réseau, aims to provide a real-time representation of the railway infrastructure, facilitating efficient synchronization with other transportation modes such as road, maritime, and inland navigation. By integrating a Service-Oriented Architecture (SOA), the Digital Twin allows seamless data sharing among stakeholders—including infrastructure managers, logistics companies, and transportation operators—enabling effective multimodal transportation planning and management. The DT centralizes all the data related to the railway network, offering a unified and accurate source of information, thereby optimizing the coordination and execution of multimodal freight transport. This approach not only promotes the decarbonization of transportation but also enhances the efficiency and resilience of the entire freight transportation system. By using the DT, the paper highlights its significant role in supporting a modal shift toward more sustainable options, like rail, thus contributing to the reduction of greenhouse gas emissions in line with environmental goals.

\citet{dorofeev2024improving} discusses the role of Digital Twins (DT) in improving Transportation Management Systems (TMSs) for freight transport reliability. A Digital Twin of an Organization (DTO) is proposed to enhance the management of business processes involved in transportation. The DTO is built using ontological modeling and Process Mining techniques, which help in reconstructing business processes from event logs and identifying deviations that could impact transport reliability. This approach supports freight transportation by providing a real-time, virtual representation of an organization's operations, enabling proactive identification and correction of deviations. Digital Twins integrate data from GPS/GLONASS systems, IoT sensors, and TMS event logs to create a synchronized digital environment that mimics the physical processes. This integration allows for better decision-making, improved route planning, and real-time monitoring, ultimately enhancing the reliability and efficiency of the freight transportation system, particularly by reducing delays and improving cargo safety. The Digital Twin concept thus ensures that transportation companies can adapt to changes and optimize their logistics processes to meet customer expectations consistently.

\citet{sun2024enhancing} presents the use of Digital Twin (DT) technology to enhance transportation efficiency in shipyards through dynamic scheduling of multiple transporters. The DT creates a real-time virtual model of the shipyard environment, integrating real-time data from physical transporters and blocks, which enables precise mapping and synchronization between the physical and digital spaces. This integration allows for optimized scheduling and allocation of transporters, addressing challenges such as road restrictions and irregular block shapes. By utilizing Geographic Information Systems (GIS), sensors, and data-driven optimization techniques, DT technology enables the simulation and proactive management of the transportation process, improving the efficiency of block movement and reducing delays. The dynamic scheduling framework of DT allows for continuous feedback between the physical and virtual models, helping to quickly adapt to any disruptions and minimizing idle times. As a result, DT technology significantly enhances freight transportation by ensuring optimal use of resources, reducing operational costs, and improving the overall shipbuilding process by streamlining operations and improving coordination among stakeholders. 

